Offline-to-online Reinforcement Learning for Image-based Grasping with Scarce Demonstrations

Offline-to-online reinforcement learning (O2O RL) aims to obtain a continually improving policy as it interacts with the environment, while ensuring the initial policy behaviour is satisficing. This satisficing behaviour is necessary for robotic manipulation where random exploration can be costly due to catastrophic failures and time. O2O RL is especially compelling when we can only obtain a scarce amount of (potentially suboptimal) demonstrations$\unicode{x2014}$a scenario where behavioural cloning (BC) is known to suffer from distribution shift. Previous works have outlined the challenges in applying O2O RL algorithms under the image-based environments. In this work, we propose a novel O2O RL algorithm that can learn in a real-life image-based robotic vacuum grasping task with a small number of demonstrations where BC fails majority of the time. The proposed algorithm replaces the target network in off-policy actor-critic algorithms with a regularization technique inspired by neural tangent kernel. We demonstrate that the proposed algorithm can reach above 90\% success rate in under two hours of interaction time, with only 50 human demonstrations, while BC and existing commonly-used RL algorithms fail to achieve similar performance.

==> sections/outline.tex <==
\section{Paper Outline}
Contributions:
\begin{enumerate}
    \item Demonstrate offline fails with a simple real-life reacher task with images, but still fine with state-based observations
    \item An algorithm that simplifies Q-learning with the NTK augmentation and self-imitation learning
    \item An experiment where we can do real-life image-based grasping in reasonable amount of time
    \item Analysis on vision backbone being unnecessary
    \item Some ablation on whether this is truly minimal setup
    \item Visualization on what's going on with the models
\end{enumerate}

Algorithm:
\begin{enumerate}
    \item Dropped target network and double-Q, replaced with a latent representation regularizer $\Phi(s, a) \Phi(s, a)^\top$.
    \item The pessimistic regularizer takes minimum return into consideration, i.e. $(Q(s, a) - \min Q)^2$, where $a \sim \cU(\cA)$.
    This is further weighted by a Gaussian kernel.
    \item Self imitation learning
    \item 3-step return
\end{enumerate}

Optional:
\begin{enumerate}
    \item End-to-end training
    \item Pretrain vision backbone (e.g. HILP)
\end{enumerate}
This mostly trades off the training speed (in wall time) while potentially decreasing asymptotic performance.

Ablations:
\begin{enumerate}
    \item Env: Pick task
    \item Algorithms:
    \begin{enumerate}
        \item Ours
        \item Cross-Q
        \item SAC (i.e. Target network)
        \item BC
        \item Self imitation learning ablation
        \item 1-step ablation
        \item Uniform OOD vs Policy OOD
        \item Gaussian weighted vs Uniform weighted
    \end{enumerate}
\end{enumerate}

Plots:
\begin{enumerate}
    \item Plot using policy action vs uniform action
    \item Plot latent representation from HILP vs from scratch
\end{enumerate}
